Simulating hydromagnetic processes in star formation: introducing ambipolar diffusion into an adaptive mesh refinement code

Given the importance of simulating hydromagnetic processes that impact star formation, we have earlier developed a 3D adaptive mesh approach that allows us to include hydromagnetic processes during the formation and evolution of cores, discs, and stars in observed regions of star formation. In this paper, we take the next step in this program - namely - to develop a modified version of the 3D adaptive mesh refinement (AMR) code FLASH in which the ambipolar diffusion of the magnetic field in poorly ionized molecular gas is implemented. We approach the problem using a single-fluid approximation to simplify numerical calculations. In this paper, we present a series of test cases including oblique isothermal and non--isothermal C-shocks. We also present a study of the quasi-static collapse of an initial uniform, self-gravitating, magnetized sphere that is initially supported by its magnetic field against collapse (i.e. magnetically subcritical). Applications to the collapse of a pre-stellar Bonnor-Ebert sphere are presented in a companion paper.

==> images/eps2pdf <==
#!/bin/sh
#
# The eps2pdf script uses ghostscript to convert eps files to pdf.
#
# Wouter Kager, 2007/06/01

program=`basename $0`
gsopts="-q -dSAFER -dNOPAUSE -dBATCH"
force=n
dres=
fixbb=n
model=
quality=
angle=0
xscale=1
yscale=1
width=
height=

echo "$program 2007/06/01 by Wouter Kager"
echo

# Scan command line options.
while getopts :Bd:fh:j:m:r:s:w: optionkey $*; do
	case $optionkey in
		B)	fixbb=y ;;
		d)	dres=$OPTARG ;;
		f)	force=y ;;
		h)	height=`echo "$OPTARG" | sed 's/[0-9\.]*/& /'` ;;
		j)	quality=`expr 100 - $OPTARG` ;;
		m)	if [ $OPTARG != CMYK -a $OPTARG != RGB -a $OPTARG != Gray ]; then
				echo "$program: invalid color model requested!"
				echo "$program: run $program without arguments for help"
				exit 1
			fi
			model="-dProcessColorModel=/Device$OPTARG" ;;
		r)	angle=$OPTARG ;;
		s)	xscale=`echo $OPTARG,$OPTARG | cut -d , -f 1`
			yscale=`echo $OPTARG,$OPTARG | cut -d , -f 2` ;;
		w)	width=`echo "$OPTARG" | sed 's/[0-9\.]*/& /'` ;;
		:)	echo "$program: the option -$OPTARG requires an argument!"
			echo "$program: run $program without arguments for help"
			exit 1 ;;
		?)	echo "$program: the option -$OPTARG is illegal!"
			echo "$program: run $program without arguments for help"
			exit 1 ;;
	esac
done

shift `expr $OPTIND - 1`

# Check if we have received any input files.
if [ ${#} -eq 0 ]; then
	cat <<-EOF
		Usage: $program [options] file(s)
		
		The valid options are:
		 -B           use ghostscript to correct the Bounding Box
		 -d res       set distiller / resampling resolution (dpi)
		 -f           force files to be overwritten if they exist
		 -h height    scale image to desired height (in cm/mm/in)
		 -j quality   use jpeg compression, quality from 1 to 100
		 -m model     set color model to either RGB, CMYK or Gray
		 -r angle     rotate counter-clockwise by angle (degrees)
		 -s scale     scale image by the requested scaling factor
		 -s xs,ys     sets horizontal,vertical scaling separately
		 -w width     scale image to specific width (in cm/mm/in)
		EOF
	exit 0
fi

#--------------------------- Function definitions ---------------------------

# find_bbox scans the file $1 for the bounding box.
find_bbox ()
{
	if [ $fixbb = y ]; then
		# we try to capture parts of the image at negative coordinates too.
		set -- `gs $gsopts -sDEVICE=bbox -c "800 800 translate" -f "$1" 2>&1 |
			awk '/HiRes/ { print $4-($2),$5-($3),$2-800,$3-800 }'`
	else
		# tr removes CR characters from DOS files, and awk selects either the
		# first or the last (atend) %%BoundingBox line for the coordinates. 
		set -- `sed -n 's/^%%BoundingBox: //p' "$1" | tr -d "\r" |
			awk 'BEGIN {w=0; h=0; x=0; y=0}
			/-?[0-9]+ -?[0-9]+ -?[0-9]+ -?[0-9]+/ {
				w=$3-($1); h=$4-($2); x=$1; y=$2; if (NR==1) {exit}}
			END {print w,h,x,y}'`
	fi

	wd=$1; ht=$2; bx=$3; by=$4
}

# set_rscode sets the rotation and scaling code.
set_rscode ()
{
	rscode="/in {72 mul} def /cm {2.54 div in} def /mm {25.4 div in} def"

	if [ -n "$width" ]; then
		rscode="$rscode $width $wd div"
		if [ -n "$height" ]; then rscode="$rscode $height $ht div";
		else rscode="$rscode dup"; fi
	else
		if [ -n "$height" ]; then rscode="$rscode $height $ht div dup";
		else rscode="$rscode $xscale $yscale"; fi
	fi

	rscode="$rscode 2 copy exch $wd mul exch $ht mul add dup translate"
	rscode="$rscode $angle rotate scale $bx neg $by neg translate"
}

# new_bbox computes the new bbox after rotation and scaling.
new_bbox ()
{
	set -- `gs $gsopts -sDEVICE=bbox -c "$rscode" -f "$1" 2>&1 |
			awk '/HiRes/ { print $4-($2),$5-($3),$2,$3 }'`

	nwd=$1; nht=$2; nx=$3; ny=$4
}

# set_dp sets the distiller compression and resampling parameters.
set_dp ()
{
	gsres=
	dp="systemdict /setdistillerparams known { <<"
	dp="$dp /AutoFilterColorImages false /AntiAliasColorImages true"
	dp="$dp /AutoFilterGrayImages false /AntiAliasGrayImages true"

	if [ -n "$quality" ]; then
		dp="$dp /ColorImageFilter /DCTEncode /GrayImageFilter /DCTEncode"
		dp="$dp /ColorImageDict << /QFactor 0.$quality /ColorTransform 1"
		dp="$dp /Blend 1 /HSamples [1 1 1 1] /VSamples [1 1 1 1] >>"
		dp="$dp /GrayImageDict << /QFactor 0.$quality /ColorTransform 1"
		dp="$dp /Blend 1 /HSamples [1 1 1 1] /VSamples [1 1 1 1] >>"
	else
		dp="$dp /ColorImageFilter /FlateEncode /GrayImageFilter /FlateEncode"
	fi

	if [ -n "$dres" ]; then
		dp="$dp /DownsampleColorImages true"
		dp="$dp /ColorImageDownsampleThreshold 1.0 /ColorImageResolution $dres"
		dp="$dp /DownsampleGrayImages true"
		dp="$dp /GrayImageDownsampleThreshold 1.0 /GrayImageResolution $dres"
		gsres="-r$dres"
	fi

	dp="$dp >> setdistillerparams } if"
}

# distill uses gs to convert $1 to $base.pdf.
distill ()
{
	if [ -n "$width$height" -o $xscale$yscale != 11 -o $angle != 0 ]; then
		set_rscode
		new_bbox "$1"
		gs $gsopts $model $gsres -sDEVICE=pdfwrite -sOutputFile="$base.pdf" \
		-c "$dp" -c "<< /PageSize [$nwd $nht] >> setpagedevice" \
		-c "$nx neg $ny neg translate $rscode" -f "$1" -c quit > $tmp.log 2>&1
	else
		gs $gsopts $model $gsres -sDEVICE=pdfwrite -sOutputFile="$base.pdf" \
		-c "$dp" -c "<< /PageSize [$wd $ht] >> setpagedevice" \
		-c "$bx neg $by neg translate" -f "$1" -c quit > $tmp.log 2>&1
	fi
}

# show_error reports errors after running $1.
show_error ()
{
	echo [error]
	echo "$program: $1 reported the following errors:"
	echo
	cat $tmp.log
}

# ------------------------ End of function definitions ----------------------

tmp=$program$$
OK=y

# Make sure existing files are only overwritten if the user agrees.
if [ -w $tmp.log -a $force = n ]; then
	echo "$program: warning, the file $tmp.log exists!"
	printf "$program: should I overwrite it (y/n)? "
	read OK

	if [ "$OK" != y ]; then
		echo "$program: in that case, I can't proceed"
		exit 0
	fi
fi

# Set the distiller parameters.
set_dp

# Loop through all files specified on the command line.
for file
do

echo
base=`echo "$file" | sed 's/\.eps$//'`

# See if the input file is there.
if [ ! -f "$base.eps" ]; then
	echo "$program: file $base.eps: no such file (skipping)"
	continue
fi
if [ ! -r "$base.eps" ]; then
	echo "$program: file $base.eps: not readable (skipping)"
	continue
fi

echo "$program: processing file $base.eps"

# Find bounding box.
find_bbox "$base.eps"
if [ $wd = 0 -o $ht = 0 ]; then
	echo "$program: no bounding box found (skipping)"
	continue
fi

# Only overwrite existing pdf file if the user agrees.
if [ -w "$base.pdf" -a $force = n ]; then
	echo "$program: warning, the file $base.pdf exists!"
	printf "$program: should I overwrite it (y/n)? "
	read OK
fi

# Perform the conversion or skip the file.
if [ "$OK" = y ]; then
	printf "$program: $base.eps -> $base.pdf "

	distill "$base.eps"
	if [ $? -ne 0 ]; then show_error "gs distiller"; continue; fi

	echo [ok]
else
	echo "$program: file $base.eps skipped [ok]"
fi

done

# Clean up.
rm -f $tmp.log

